Membership Inference Attacks and Defenses in Classification Models

We study the membership inference (MI) attack against classifiers, where the attacker's goal is to determine whether a data instance was used for training the classifier. Through systematic cataloging of existing MI attacks and extensive experimental evaluations of them, we find that a model's vulnerability to MI attacks is tightly related to the generalization gap -- the difference between training accuracy and test accuracy. We then propose a defense against MI attacks that aims to close the gap by intentionally reduces the training accuracy. More specifically, the training process attempts to match the training and validation accuracies, by means of a new {\em set regularizer} using the Maximum Mean Discrepancy between the softmax output empirical distributions of the training and validation sets. Our experimental results show that combining this approach with another simple defense (mix-up training) significantly improves state-of-the-art defense against MI attacks, with minimal impact on testing accuracy.

==> 0_eval.tex <==

\begin{comment}

\mypara{Revisions}
\begin{itemize}
    \item 
Revise the paper to reflect the fact that baseline attack is already in Yoem et al.
    \item
Explore whether it is possible to explain the empirical observation that the advantage of best attack is bounded by double that of the baseline attack?  Suppose we assume that the model results in probabilities following some distribution (Gaussian), can we show that things cannot be distinguished? 
    \item
See whether it is possible to perform attack without training any shadow models, and purely based on model outputs of a set of instances, where it is known that some percentage are used in training, although which ones are used is unknown.  
    \item
Compare the defense mechanism of reducing training-testing gap with other defence methods explored in the submission.
    \item
Expirically compare the approach of using DP to train the model with other defenses. 
    \item
Assume trained model parameters follow the exponential distribution.  Instances used in training and not in training follow IID.  Their lose function should follow two distributions (beta with different parameters).  That may explain the bounding gap.
\end{itemize}

%\input{hyptheory.tex} 
\end{comment}

\subsection{Discussions}

     
\begin{comment}
    %\begin{figure}[h]
    %\centering
    %\includegraphics[width=9cm,height=8cm]{figures/freeze.pdf}
    %\caption{The effect of number of frozen layers on training accuracy and testing accuracy. %ResNet-18/VGG-16 on CIFAR-10/CIFAR-100 dataset. $50,000$ training instances are used. We got %similar results on other neural network architectures we use in this paper.}
    %\label{freeze}
    %\end{figure}
    
     
     Since we choose the classifiers pre-trained on ImageNet, we need to change the last several layers for those pre-trained classifiers to be compatible with CIFAR-10 or CIFAR-100 dataset. The details of modification of each network are described in Appendix. When fine-tuning pre-trained classifiers, one needs to consider how many layers are frozen. In \cite{yosinski2014transferable}, experimental results show that if we only freeze the first several layers, the final testing accuracy remains similar.  We also investigated what is the best choice when selecting the number of frozen layers in our case. As shown in Figure \ref{freeze}, if we do not freeze any layer, the testing accuracy will be similar to the optimal choice. From the classification task perspective, only the classifier with best testing accuracy will be deployed in practical scenarios, which makes no frozen layers a good choice. When taking MI attacks into consideration, since we want to evaluate fine-tuning as a defense, we want to evaluate the case where the target classifier is as vulnerable as possible, while the testing accuracy is maintained. If none of the layers is frozen, then it is the easiest situation for the target classifier to overfit the fine-tuning set because all the parameters can be changed. This setting makes it easier to launch MI attacks. Thus, we analyze our attack and defense \textbf{without freezing any layer} when fine-tuning in the following experiments. The learning rate is 0.0005 when using pre-trained classifier and the training epoch is one half of the epochs when training from scratch.
     
     For mix-up defense, we adopt the code from the public repository by the author of \cite{zhang2018mixup}. 
     %Notice that the ResNet-18, ResNet-101 and DenseNet-121 were designed for ImageNet dataset with kernel size of $7*7$ in the first convolutional layer. In our experiment, we do not modify the the kernel size of the first convolutional layer and this leads to worse testing accuracy than ResNet-20, ResNet-110 and DenseNet\_BC(100,12), which were designed for CIFAR dataset with $3*3$ kernel size in the first convolutional layer.
\end{comment}
    
     %For PURCHASE-100 and TEXAS-100, there is no pre-trained classifier for them, since they are not image data. 
     For PURCHASE-100 and TEXAS-100 dataset, we observed that using mix-up training leads to training failure.  Perhaps this is due to the fact that the data features are binary.  We thus do not evaluate these two defenses on them. The only applicable defense is the MMD loss defense.
     
%     Again, any method that can close the generalization gap would offer improved defense against MI attacks, such as using available pre-trained classifiers.
    
    
    %Our training data size $|D|$ is fixed to 10000 when testing different attacks, which is less than one half of the original training set size in CIFAR-10 and CIFAR-100. For PURCHASE-100 dataset, we use $|D|=20000$ and $|D|=10000$ for TEXAS-100 dataset. For MNIST dataset, we also use $|D|=10000$.
    
    %\textbf{Traditional machine learning algorithms}. We use algorithms implemented in scikit-learn \cite{scikit-learn} to train our target classifiers. Four types of machine learning classifiers (logistic regression, k-nearest neighbor, decision tree and Naive Bayes) will be utilized as our target classifiers.

%    \mypara{Attack models.} We use logistic regression classifier implemented in scikit-learn \cite{scikit-learn} as our attack model for our Instance-Probability attack in this paper.  For all the previous proposed attacks, we follow the attack model proposed in the original papers for evaluation.

    
\subsection{Evaluation of Defenses} \label{sec:defense_eval}
 
Tables~\ref{defense_avg_cifar10} and \ref{defense_avg_cifar100} give the numbers averaged across the classifiers with different level of defenses. Figure ~\ref{fig:defense} shows the effect of different level of defenses on different classifier and dataset combinations. Notice that in Figure ~\ref{fig:defense}, only generalization gap, the baseline attack advantage and the largest attack advantage are reported for each dataset, network and defense level combination.
    
One main observation is that using MMD loss or mix-up alone each offers some reduction in generalization gap; and combining mix-up with MMD loss offers better defense.  However, the generalization gap are not fully closed by the defense.  With both defense, the largest attack advantage in CIFAR-10 decrease from 0.173 to 0.092, and that for CIFAR-100 decreases from 0.362 to 0.147. 


%For those classifiers which have pre-trained classifiers available, the largest attack advantage can be further decreased, as shown in Figure ~\ref{fig:transfer_defense}.  With all defense deployed, he largest attack advantage in CIFAR-10 decrease from 0.213 to 0.081, and that for CIFAR-100 decreases from 0.421 to 0.183 (averaging across VGG-16, ResNet-18 and DenseNet-121).


\begin{comment}

    \begin{figure}
        \centering
        \includegraphics[width=9cm,height=5cm]{figures/transfer-defense.pdf}
        \caption{Attack advantage of different attacks for different classifiers on different datasets with different level of defenses. DEF1 means no defense, DEF2 means mix-up defense, DEF3 means MMD loss\&mix-up defense and DEF4 means MMD loss \&mix-up\&fine-tuning defense.}
        \label{fig:transfer_defense}
    \end{figure}
    
\end{comment}
 

Another observation is that with both MMD loss and mix-up, most attacks in the literature become a lot less effective and perform similar to the baseline. 
    
Our proposed Instance-Probability attack performs the best.  Interestingly, the Instance-Vector attack, which performs significantly worse than other attacks on CIFAR-10 and CIFAR-100 when no defense is used, perform close to the Instance-Probability attack with both defences.  It appears that when evaluating defence effectiveness, one needs to consider Instance-level attacks.  If we were to consider only the Class-Vector attack, we would have concluded that the proposed defenses are highly effective, since its advantage is greatly reduced. 
    
Perhaps the most important finding from these experimental results is that the relationship  $\frac{g}{2} \le v \le g$ remains valid in all experiments with different kinds of defenses.  
   %This suggests that the problem of defending against MI attacks is largely the task of the ML research community, whose main goal is to design methods to train classifiers that generalize well.  At the same time, we need to examine whether more effective MI attacks exist.  
     %since closing the generalization gap is already the goal of ML.  The research community can focus on the goal of developing techniques to train better classifiers, and the threat of black-box MI attacks is taken care of as a side effect.  This is not the case for some other security/privacy problems of ML, such as adversary examples and poisoned training. 
     
Regarding Purchase-100 dataset and Texas-100 dataset, the only applicable defense is the MMD-loss defense. With MMD-loss defense deployed, we see that the largest attack advantage drops from 0.140 to 0.089 and from 0.178 to 0.146. 
%\textcolor{red}{do we need to add some comments for this?}

\begin{comment}

\begin{table*}
    \centering
    \begin{tabular}{lrrr}
        %\hline
        Defense level & No Defense & Mixup+MMD loss defense  & Mem-Guard Defense\\
        \toprule
        %\hline
        Training accuracy & 0.994 & {\bf 0.881} & 0.997\\
        %\hline
        Testing accuracy &  0.761 & {\bf 0.765} & 0.762\\
       % \hline
    %    \hline
       \cmidrule(lr){1-4}
        \textbf{Generalization gap} & 0.232  & {\bf 0.116} & 0.235 \\
        %\hline
        \textbf{Largest attack advantage} & 0.166 & {\bf 0.067} & 0.113 \\
      %  \hline
        \textbf{Baseline attack advantage} & 0.116 & {\bf 0.067} & 0.112 \\
        %\hline
        %\hline
               \cmidrule(lr){1-4}
        Global-Probability attack advantage & 0.156 & {\bf 0.067} & 0.112\\
        Global-Loss attack advantage & 0.166 & {\bf 0.056} & 0.113 \\
        %\hline
        Global-TopOne attack advantage & 0.120 & 0.049 & {\bf 0.028}\\
        %\hline
        Global-TopThree attack advantage & 0.140 & 0.052 & {\bf 0.027}\\
        %\hline
        Class-Vector attack advantage & 0.137 & {\bf 0.054} & 0.113\\
       % \hline
       \bottomrule
    \end{tabular}
    \caption{Our MI defense significantly outperforms the Mem-Guard defense~\cite{jia2019memguard} on the CIFAR-10 dataset with Alexnet, VGG-16 and ResNet-20. The numbers are averaged across the three neural networks.}
    \label{tab:memguard_cifar10}
\end{table*}

\end{comment}


\begin{table*}
    \centering
    \begin{tabular}{lrrrrrr}
        \multicolumn{1}{c}{Dataset} & \multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        %\hline
         Defense level & No Def. &  Mixup+MMD & Mem-Guard & No Def. & Mixup+MMD  & Mem-Guard \\
        \cmidrule(lr){1-4}
        \cmidrule(lr){4-7}
        %\hline
        Training accuracy & 0.994 & {\bf 0.881} & 0.997 & 0.995 & {\bf 0.665} & 0.979 \\
        %\hline
        Testing accuracy &  0.761 & {\bf 0.765} & 0.762 & 0.326 & {\bf 0.337} & {\bf 0.338}\\
       % \hline
    %    \hline
        \cmidrule(lr){1-4}
        \cmidrule(lr){4-7}
        \textbf{Generalization gap} & 0.232  & {\bf 0.116} & 0.235  & 0.669 & {\bf 0.328} & 0.641\\
        %\hline
        \textbf{Largest attack advantage} & 0.166 & {\bf 0.067} & 0.113 & 0.356 & {\bf 0.166} & 0.324\\
      %  \hline
        \textbf{Baseline attack advantage} & 0.116 & {\bf 0.067} & 0.112 & 0.333 & {\bf 0.166} & 0.324\\
        %\hline
        %\hline
        \cmidrule(lr){1-4}
        \cmidrule(lr){4-7}
        Global-Probability attack advantage & 0.156 & {\bf 0.067} & 0.112 & 0.356 & {\bf 0.166} & 0.320\\
        Global-Loss attack advantage & 0.166 & {\bf 0.056} & 0.113 & 0.356 & {\bf 0.155} & 0.319\\
        %\hline
        Global-TopOne attack advantage & 0.120 & 0.049 & {\bf 0.028} & 0.249 & 0.103 & {\bf 0.093}\\
        %\hline
        Global-TopThree attack advantage & 0.140 & 0.052 & {\bf 0.027}  & 0.273 & 0.104 & {\bf 0.063}\\
        %\hline
        Class-Vector attack advantage & 0.137 & {\bf 0.054} & 0.113 & 0.320 &  {\bf 0.115} & 0.316\\
       % \hline
       \bottomrule
    \end{tabular}
    \caption{Our MMD+Mix-up MI defense significantly outperforms the Mem-Guard defense~\cite{jia2019memguard} on the CIFAR-10 and CIFAR-100 dataset using Alexnet, VGG-16 and ResNet-20 CNNs. The numbers are averaged across the three neural networks.}
    \label{tab:memguard_cifar10}
\end{table*}

%\vspace{-3em}
\begin{comment}
\begin{table*}
    \centering
    \begin{tabular}{lrrr}
        %\hline
        Defense level & No Defense  & Mixup+MMD loss defense & Mem-Guard Defense\\
        \toprule
        %\hline
        Training accuracy & 0.995 & {\bf 0.665} & 0.979 \\
        %\hline
        Testing accuracy & 0.326 & {\bf 0.337} & {\bf 0.338}\\
        %\hline
        %\hline
        \cmidrule(lr){1-4}
        \textbf{Generalization gap} & 0.669 & {\bf 0.328} & 0.641 \\
        %\hline
        \textbf{Largest attack advantage} & 0.356 & {\bf 0.166} & 0.324\\
        %\hline
        \textbf{Baseline attack advantage} & 0.333 & {\bf 0.166} & 0.324\\
        %\hline
        %\hline
        \cmidrule(lr){1-4}
        Global-Probability attack advantage & 0.356 & {\bf 0.166} & 0.320\\
        
        Global-Loss attack advantage & 0.356 & {\bf 0.155} & 0.319\\
        %\hline
        Global-TopOne attack advantage & 0.249 & 0.103 & {\bf 0.093}\\
        %\hline
        Global-TopThree attack advantage & 0.273 & 0.104 & {\bf 0.063}\\
        %\hline
        Class-Vector attack advantage & 0.320 &  {\bf 0.115} & 0.316\\
        %\hline
        \bottomrule
    \end{tabular}
    \caption{Our MI defense significantly outperforms the Mem-Guard defense~\cite{jia2019memguard} on the CIFAR-100 dataset with Alexnet, VGG-16 and ResNet-20. The numbers are averaged across the three neural networks.}
    \label{tab:memguard_cifar100}
\end{table*}
\end{comment}


\subsection{Comparison against Existing Defenses}\label{sec:eval:memguard}
In this section, we compare our defense with existing defenses. 
%Comparison with differential privacy will be discussed in the next section.

In modern deep neural network training, $L_2$-regularizer and dropout is widely used. In our experiment, we already use these two techniques during the training, thus we don't compare our defense with these two. 
 %We also do not consider classifier stacking defense here because multiple classifiers are used in classifier stacking and we only consider a single classifier case throughout the whole evaluation. 
Model stacking, according to~\cite{jia2019memguard}, will incur high label loss, which implies high testing accuracy drop.  In this paper, we focus on defenses that are able to maintain the testing accuracy while defending the membership inference attack.  

According to~\cite{jia2019memguard}, the Mem-Guard defense could outperform all existing defenses including MIN-MAX Game defense~\cite{nasr2018machine}, here we focus our comparison with Mem-Guard. 
We adopt the code from ~\cite{jia2019memguard} and use default parameters. In our experiment, we test Baseline attack, Global-Probability attack, Global-Loss attack, Global-TopOne attack, Global-TopThree attack and Class-Vector attack against Mem-Guard.  We exclude the two instance level attack here because training a model with Mem-Guard is slow, and we need to train 50 shadow classifiers to learn instance-specific information.  
Even for a small CNN like Alexnet, it takes 14 hours to train one Alexnet classifier on CIFAR-10 with <em-Guard.  For comparison, it takes 20 minutes to train one Alexnet classifier with our MMD+Mix-up defense.  

For the same reason, when comparing with Mem-Guard, we use only three of the seven NN architectures  used in earlier evaluations.  
 %Mem-Guard still takes more than one month of GPU time to evaluate the instance level attacks (which requires training 50 shadow classifiers to learn instance-specific information). In contrast, learning our MMD+Mix-up defense takes on Alexnet over all seven attacks takes only 17 GPU hours. 
 %We use the probability vectors defended by Mem-Guard, i.e. the predictions with noise generated by Mem-Guard, to evaluate the attacks. 
More specifically, we use AlexNet, VGG-16 and ResNet-20 on CIFAR-10 and CIFAR-100 dataset. We chose these three because they are small, and faster to train with Mem-Guard.

The results (averaged over AlexNet, VGG-16 and ResNet-20) are shown in Table ~\ref{tab:memguard_cifar10}. We see that Mem-Guard defense can fully defend Global-TopOne attack and Global-TopThree attack. However, when it comes to Global-Probability attack and Class-Vector attack, Mem-Guard defense can only reduce the attack advantages of these two attack to the attack advantage of baseline attack. Mem-Guard has no impact on the baseline attack, since it does not reduce the generalization gap. 
 %One important observation for Mem-guard defense and MIN-MAX Game defense is that the generalization gap is not considered and the training accuracy is close to 1 almost for all cases. It is easy to see that their defense cannot defend against baseline attack.
Our defense, which focus on reducing the generalization gap, provides better defense since the largest attack advantage under our defense is lower than the largest attack advantage under Mem-Guard defense by a noticeable margin (0.046 for CIFAR-10 and 0.158 for CIFAR-100).

%We also observe partial failure of defense on VGG-16 using Mem-Guard, meaning that for 23\% of the instances, no noise can be found to fool the defender's attack classifier.
%One important piece of information ignored by Mem-Guard defense is the true label of instance and intuitively this is the reason why Baseline attack, Global-Probability attack and Class-Vector attack can still work against Mem-Guard defense. 

Differential privacy offers a principled defense against MI attacks, in the sense that the $\epsilon$ parameter determines an upperbound on the advantage of any possible MI attacks.
However, current techniques for satisfying DP do not yet offer practically effective defense against MI attacks.  Existing techniques incur heavy cost in terms of testing accuracy.  For example, as reported in \cite{abadi2016deep}, when the privacy budget is $\epsilon=\{2,4,8\}$, the test accuracy (trained using all data) is $\{67\%,70\%,73\%\}$ on CIFAR-10 dataset. The test accuracy without differential privacy guarantee is $86\%$ using an architecture similar to \cite{abadi2016deep}, and over 95\% using DenseNet.  

\textcolor{red}{To validate that our method is better than DP-SGD, we compare our MMD+Mix-up defense with DP-SGD in two ways: 1. training accuracy vs testing accuracy; 2. testing accuracy vs best attack advantage. As shown in Figure \ref{fig:dpsgd_training_testing_acc}, the generalization gap when training using our method is smaller than the generalization gap when training using DP-SGD. One needs to notice that, in order to achieve comparable testing accuracy, the privacy budget is significantly larger than standard choice. Smaller generalization gap means smaller highest attack advantage, as shown in Figure \ref{fig:dpsgd_attack_advantage}. When the testing accuracy is the same, our method can give better defense than DP-SGD, which results in smaller highest attack advantage. By the two figures above, we can summarize that our MMD+Mix-up defense can provide better utility-privacy trade-off. One more thing we want to point out is that, even though we use extraordinarily high privacy budget, the highest attack advantage 
is still bounded by the generalization gap, meaning that we still need to investigate more powerful attacks.}

From the perspective of privacy, one should note that $\epsilon=1$ ensures a theoretical upperbound of $\frac{e}{1+e}-0.5\approx 0.23$ on MI advantage, and $\epsilon=2$ yields a theoretical upperbound of $0.38$.  In contrast, while our defenses are deployed, the largest attack advantage is 0.093 and 0.168 for CIFAR-10 dataset and CIFAR-100 dataset, respectively.


\subsection{Validation set membership inference}
\textcolor{red}{
We utilize a set of validation data to compute the MMD loss during training and this may raise the question that the trained model may overfit the validation data and thus leak the membership information of the validation set. To address this issue, we keep the same experimental setting and launch the membership inference attack against the validation set. However, the best attack advantage we can have is less than $2\%$ among all different models and datasets.
}

\subsection{When the evaluation set is not balanced}
When the MI attack evaluation set is not balanced, what will happen?

 %What should we say between our defense and dp?

%Further, $\epsilon=2$ ensures an upperbound of $\frac{e^2}{1+e^2}-0.5\approx 0.38$, and $\epsilon=3$ ensures an upperbound of $\frac{e^3}{1+e^3}-0.5\approx 0.45$.  For comparison, the highest MI advantage we observe in experiments without defense is around 0.43 for CIFAR-100 on DenseNet-121.  At the same time, an $\epsilon$ value of $1$ to $3$ is quite common in the literature on DP; and some papers use $\epsilon$ value in the hundreds or thousands.  







 \begin{table*}
    \normalsize
     \centering
     \begin{center}
    \begin{tabular}{lrrrrrr}
        %\multicolumn{1}{c}{Dataset } & \multicolumn{3}{c}{CIFAR-10} & %\multicolumn{3}{c}{CIFAR-100} \\
        %\cmidrule(lr){1-1}
        %\cmidrule(lr){2-4}
        %\cmidrule(lr){5-7}
        
        \multicolumn{1}{c}{Dataset-Model}  & \multicolumn{3}{c}{No Defense} & \multicolumn{3}{c}{MMD \& mix-up defense} \\
        
        \multicolumn{1}{c}{-} & Testing Acc. & Best Attk. Advantage & Gap  & Testing Acc. & Best Attk. Advantage & Gap \\
        
        
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        
        
        \multicolumn{1}{c}{CIFAR-10 - Alexnet} & \multicolumn{1}{c}{0.652} & \multicolumn{1}{c}{0.210} & \multicolumn{1}{c}{0.337} & \multicolumn{1}{c}{0.682} & \multicolumn{1}{c}{0.132} & \multicolumn{1}{c}{0.142}\\
        
        \multicolumn{1}{c}{CIFAR-10 - VGG-16} & \multicolumn{1}{c}{0.811} & \multicolumn{1}{c}{0.162} & \multicolumn{1}{c}{0.169} & \multicolumn{1}{c}{0.809} & \multicolumn{1}{c}{0.097} & \multicolumn{1}{c}{0.108} \\
        
        \multicolumn{1}{c}{CIFAR-10 - ResNet-20} & \multicolumn{1}{c}{0.820} & \multicolumn{1}{c}{0.130}& \multicolumn{1}{c}{0.171}& \multicolumn{1}{c}{0.818}& \multicolumn{1}{c}{0.086}& \multicolumn{1}{c}{0.106}\\
        
        \multicolumn{1}{c}{CIFAR-10 - ResNet-110} & \multicolumn{1}{c}{0.794}& \multicolumn{1}{c}{0.130}& \multicolumn{1}{c}{0.171}& \multicolumn{1}{c}{0.784}& \multicolumn{1}{c}{0.084}& \multicolumn{1}{c}{0.106}\\
        
        \multicolumn{1}{c}{CIFAR-10 - DenseNet-BC (100,12)} & \multicolumn{1}{c}{0.801}& \multicolumn{1}{c}{0.137}& \multicolumn{1}{c}{0.196}& \multicolumn{1}{c}{0.802}& \multicolumn{1}{c}{0.047}& \multicolumn{1}{c}{0.077}\\
        
        \multicolumn{1}{c}{CIFAR-100 - Alexnet} & \multicolumn{1}{c}{0.248}& \multicolumn{1}{c}{0.284}& \multicolumn{1}{c}{0.751}& \multicolumn{1}{c}{0.238}& \multicolumn{1}{c}{0.071}& \multicolumn{1}{c}{0.121}\\
        
        \multicolumn{1}{c}{CIFAR-100 - VGG-16} & \multicolumn{1}{c}{0.285}& \multicolumn{1}{c}{0.411}& \multicolumn{1}{c}{0.815}& \multicolumn{1}{c}{0.275}& \multicolumn{1}{c}{0.300}& \multicolumn{1}{c}{0.542}\\
        
        \multicolumn{1}{c}{CIFAR-100 - ResNet-20} & \multicolumn{1}{c}{0.446}& \multicolumn{1}{c}{0.294}& \multicolumn{1}{c}{0.542}& \multicolumn{1}{c}{0.410}& \multicolumn{1}{c}{0.072}& \multicolumn{1}{c}{0.114}\\
        
        \multicolumn{1}{c}{CIFAR-100 - ResNet-110} & \multicolumn{1}{c}{0.424}& \multicolumn{1}{c}{0.342}& \multicolumn{1}{c}{0.574}& \multicolumn{1}{c}{0.426}& \multicolumn{1}{c}{0.145}& \multicolumn{1}{c}{0.243}\\
        
        \multicolumn{1}{c}{CIFAR-100 - DenseNet-BC (100,12)} & \multicolumn{1}{c}{0.428}& \multicolumn{1}{c}{0.256}& \multicolumn{1}{c}{0.511}& \multicolumn{1}{c}{0.410}& \multicolumn{1}{c}{0.074}& \multicolumn{1}{c}{0.121}\\
        
        \multicolumn{1}{c}{Purchase - Purchase} & \multicolumn{1}{c}{0.791}& \multicolumn{1}{c}{0.142}& \multicolumn{1}{c}{0.191}& \multicolumn{1}{c}{0.781}& \multicolumn{1}{c}{0.089}& \multicolumn{1}{c}{0.152}\\
        
        \multicolumn{1}{c}{Texas - Texas} & \multicolumn{1}{c}{0.485}& \multicolumn{1}{c}{0.191}& \multicolumn{1}{c}{0.292}& \multicolumn{1}{c}{0.481}& \multicolumn{1}{c}{0.151}& \multicolumn{1}{c}{0.241}\\
        
        
       \bottomrule
    \end{tabular}
    \end{center}
     \caption{Evaluation of different attacks on different dataset and models with or without our proposed defense.}
     %\label{tab:defense_summary}
 \end{table*}
 

==> 5_discussion.tex <==


\section{Relationship with Differential Privacy} \label{sec:discussion}

%We first discuss some possible reasons for the empirical relationship that the maximum MI attack advantage is bounded by the generation gap, and then discuss the relationship between MI attacks and differential privacy. 

\begin{comment}

\begin{figure}
    \centering
    \includegraphics[width=8cm,height=4cm]{figures/cdf-labelp.eps}
    \caption{Cumulative distribution function of probability corresponding to the true label for members and non-members, on 4 different datasets. }
    \label{cdf-labelp}
\end{figure}

\subsection{Relationship of MI and generalization gap}

Here we offer an informal discussion of what led to the empirical relationship of $ v \le g$.  We plot in Figure~\ref{cdf-labelp} the cumulative probability of $(F^T(x))_y$, the probability of the true label $y$ for the members and non-members, for 4 datasets. 
$F^T$ makes correct prediction on $(x,y)$ if $(F^T(x))_y$ is higher than $(F^T(x))_{y'}$ for any other $y'$. 
When there are only 2 classes, $F^T$ would predict label $y$ when $(F^T(x))_y>0.5$.  When there are many classes, $F^T$ would predict $y$ even when $(F^T(x))_y<0.5$.  We conjecture that 

which is likely to happen when $(F^T(x))_y$ is higher than some threshold $p$, where $p$ depends on the models but .  The generalization gap is thus corresponding 

Accuracy is the probability that the true label $y$ of a random example $x$ in a given dataset is the most likely class in the probability vector $F^T(x)$.
The generalization gap is a difference in accuracy between the training $D_\text{Tr}$ and test $D_\text{Te}$ datasets. 

Note that the accuracy (of members and non-members) is lower bounded by the gap between the CDF values at $1/c$ and one, where $c$ is the number of classes, as at values smaller than $1/c$ the true label $y$ is guaranteed to not be the predicted class.


The effect observed in Figure~\ref{fig:gapvsbset} ---where the generalization gap appears to upper bound the performance of MI attacks--- is then due to a relationship between the generalization gap and the $\mathcal{H}_1$ and $\mathcal{H}_0$ clustering performance in these datasets.
From Theorem~\ref{thm:hyp}, the MI attack success probability is upper bounded by the ability to successfully cluster the samples of $D_A$ into $\mathcal{H}_1$ and $\mathcal{H}_0$ clusters, which in Figure~\ref{cdf-labelp} is a function of the gap between the member and non-member curves.
Because of the flatness in the middle of the CDF, the gap in the CDF strongly correlates with the generalization gap, which then explains the relationship seen in Figure~\ref{fig:gapvsbset}.
Note that this is due to a peculiarity of these datasets, where the test data either looks very similar to the training ---evidenced by the sharp transition at the right of the CDF--- or not at all related ---shown by the sharp jump in the beginning of the CDF.
\bruno{any conclusions?}
\end{comment}

There is a direct connection between differential privacy~\cite{Dwo06,DMNS06} and membership inference, which has been identified in the literature~\cite{shokri2017membership}.  
In our context, an algorithm $\AA(\cdot)$ is $\epsilon$-differentially private ($\epsilon$-DP) if and only if for any two training datasets $D$ and $D'$ that differ in at most one instance, we have 
\vspace*{-0.06in}
\begin{equation*}
\forall{T\subseteq \mathit{Range}(\AA)}:\; \myPr{\AA(D) \in T} \leq e^{\epsilon}\, \myPr{\AA(D') \in T}.
\end{equation*}
Let $D$ be a dataset with an instance $(x,y)$ and $D'$ be a data in which $(x,y)$ is replaced by another instance (or simply removed).  When the training algorithm is $\epsilon$-DP, the perfect MI attacker can only rely on for each classifier $F$, which of $D$ and $D'$ have higher probability of resulting to $F$ as output.  If the classifier is more likely to be one trained from $D$, then predicts ``member''; otherwise predicts ``non-member''.  The success probability of this attack is at most $\frac{e^\epsilon}{e^\epsilon+1}$.  
Therefore, if the algorithm for training a classifier is $\epsilon$-differentially private, then there exists no MI attacker who can have an advantage $ \ge \left(\frac{e^\epsilon}{e^\epsilon+1} - \frac{1}{2}\right)$.  

Given this, it appears that a principled and promising defence against MI attacks is to use training algorithms that are $\epsilon$-DP.  Designing private training algorithms has been studied before the community is specifically interested in MI attacks~\cite{shokri2015privacy,abadi2016deep}.  This defense is effective against all possible attacks, both in the black-box setting and in the white-box setting (where the adversary knows the model parameters).  Depending on how DP is guaranteed, this may be able defend against attack in the federated setting where one observes intermediate updates in the training process.  

We point out that current techniques for satisfying DP do not yet offer practically effective defense against MI attacks.  Existing techniques incur heavy cost in terms of testing accuracy.  For example, as reported in \cite{abadi2016deep}, when the privacy budget is $\epsilon=\{2,4,8\}$, the test accuracy (trained using all data) is $\{67\%,70\%,73\%\}$ on CIFAR-10 dataset. The test accuracy without differential privacy guarantee is $86\%$ using an architecture similar to \cite{abadi2016deep}, and over 95\% using DenseNet.  
 %similar to what is used in \cite{shokri2017membership}. \says{ninghui}{what dataset is it?}

Note that $\epsilon=1$ ensures a theoretical upperbound of $\frac{e}{1+e}-0.5\approx 0.23$ on MI advantage.   Coincidentally, the highest attack advantage we observe when both fine-tuning and mix-up are used is also around $0.23$ for CIFAR-100.  
Further, $\epsilon=2$ ensures an upperbound of $\frac{e^2}{1+e^2}-0.5\approx 0.38$, and $\epsilon=3$ ensures an upperbound of $\frac{e^3}{1+e^3}-0.5\approx 0.45$.  For comparison, the highest MI advantage we observe in experiments without defense is around 0.43 for CIFAR-100 on DenseNet-121.  At the same time, an $\epsilon$ value of $1$ to $3$ is quite common in the literature on DP; and some papers use $\epsilon$ value in the hundreds or thousands.  

Unless dramatic improvement in DP techniques are made, using DP to protect against MI attacks does not appear promising, when compared with defenses such as those aiming at closing the generalization gap.  However, the connection between MI attacks and DP offers another intriguing possibility.  It is highly desirable to have some confidence that an ML training algorithm satisfies DP.  Intuitively such an algorithm should not be overly dependent on any individual training instance.  Existing DP techniques show that each individual training step satisfies DP and then compose the DP parameters.  Such an analysis, however, is in some sense wasteful, since the attacker is shown only the final output, and not the outputs of the individual steps.  Due to the complexity of such training algorithms, it is desirable that there are some black-box techniques to test the privacy property of classifiers. 

MI attacks offer such a black-box test.  Li et al.~\cite{LQS+13} showed that DP is equivalent to membership privacy where the adversary's prior belief is such that the probability of any instance's membership is independent from that of any other instance.  This equivalence means that MI attack is the only attack one needs to be concerned about for testing DP properties.  
If we can prove that the advantages of all MI attacks are upper-bounded by a parameter, then the training algorithm satisfies DP.  Of course we can never enumerate through all possible MI attacks to prove this.  However, if the research community has gain in-depth understanding of MI attacks, and classifiers trained using an algorithm can resist all MI attacks (have the maximum advantage bound by some parameter), then the practical privacy consequence is equivalent to the situation that the training algorithm satisfies DP.  We point out that security guarantees of important cryptographic primitives such as block ciphers and RSA, are similarly not based on proof of security, but rather the fact that the best known attacks cannot break them.  People nonetheless have enough confidence to use them broadly, because it is believed that no adversary knows a more effective attack.  While we currently are not at a similar level of understanding regarding the threat of MI attacks on ML models, further research may lead to confidence that the community as a whole have sufficient understanding of MI attacks, so that whether an ML model resists MI attacks can be taken as an accurate indicator of its DP property. 

 %Shokri also mentioned differential privacy, which is intended to protect membership information. If the target model is trained with differential privacy technique, then the membership information should be secured. However, when the target classifier is trained with relatively small $\epsilon$, the performance of the target classifier may significantly degrade. \textcolor{red}{Need citation and further explaination.} The cost of securing membership information is too expensive to make differential privately training practical in real world application. 

 %\textbf{Differential privacy} \textcolor{red}{is a privacy preserving technique\cite{dwork2008differential}. To be more specific, suppose we have two datasets $D$ and $D'$ where these two datasets has only one instance different. Differential privacy could provide a guarantee that the output of a given algorithm on $D$ and $D'$ will be almost identical if differential privacy is applied. Differential privacy thus provide a membership protection for each instance that is possible to be used in $D$. However, when the given algorithm is a deep neural network, it is not possible to give a formal proof of membership protection even in a scenario with constraints. Thus we want to explore the membership protection that the deep neural network can intrinsically provide for each training instance.}

%\input{hyptheory}     


\begin{comment}

\subsection{future work}
    For future work, we propose two paths to explore. The first path is to adopt the research results from the area of transfer learning, which basically can exploit other public dataset to help training the model and result in better performance. By leveraging other public dataset into our training process, we both mitigate the risk of membership inference attack and improve the performance of the target model. The intuition behind is that more data is used in the training then the effect of a single data is smaller.
    
    The second path is to applying more regularization technique or better training strategy to reduce the gap between training accuracy and the testing accuracy. The better our model generalize, the less potential risk we have against membership inference attack. However, this does not imply that models do not memorize. On the contrary, better generalized model may be easier to launch the membership attack, as shown in previous section. We still need to further investigate how to better mitigate membership inference attack.



\section{Evaluation}

    We first describe the datasets we use for the evaluation of our attack, then the target model and attack model used in our experiments will be described in detail. In the following part we are going to evaluate our attack under several different settings and explain the reason why our attack works against different datasets and different machine learning algorithms.
    
    \subsubsection{Traditional machine learning algorithms as target model}

    Previous paper has suggested that the adversary could also launch membership inference attack on traditional machine learning algorithms\cite{truex2018towards}. Instead of using neural networks as our target model, we also want to explore if our attack could work on traditional machine learning algorithms such as logistic regression, k-nearest neighbor, decision tree and Naive Bayes. Thus, we follow the experiment in \cite{truex2018towards} and evaluate our attack against some traditional machine learning algorithms above on CIFAR-10 dataset. In Table \ref{traditional_attack}, we compare our attack against traditional machine learning algorithms and our attack against neural networks. Experiment data shows that some of traditional machine learning algorithms are also easy to be attacked on membership and our attack has almost the same performance as Shokri's attack when dealing with traditional algorithm. Decision tree is shown to be the most vulnerable algorithm, due to its own logic behind.  
    From our experiment, we support the idea that membership inference attack could be launched against most machine learning algorithm and the privacy of training data would be a great concern.
    

\subsection{Thinking about more challenging scenario}
    \textcolor{red}{discuss about baseline attack?}

\subsection{When and how does the memorization happen?}
    We explore more into when and how the memorization happens and we observe the correlation between the risk of membership inference attack and the gap between training accuracy and testing accuracy. As more epochs we use to train our model, higher training accuracy we will get, but this does not apply to testing accuracy. The gap between training accuracy and testing accuracy can be referred as the "generalization error" according to \cite{hardt2015train}. We observe that if the gap starts to increase, then the accuracy of membership inference attack also increases, as shown in Figure \ref{gap}. We see that when the gap between training accuracy and testing accuracy starts to increase, the membership attack accuracy of our attack and Shokri's attack both starts to increase. Generally, the gap between training accuracy and testing accuracy can be treated as a good indicator of how much the model memorizes the training instances instead of "learning".
\end{comment}


==> codaspy_rebuttal.tex <==

----------- Comments for the Authors -----------
1. There are a few minor writing errors in the paper. 
2. While the details of experiments have been made clear in the appendix, the authors should provide the code for reproducibility.

1. release code



----------- Comments for the Authors -----------
The paper is well written and covers an important topic. The range of data, ML algorithms, attacks and defenses considered is impressive. With that said, as noted above, it would be nice to see how other ML classifiers hold-up under these attacks. Also, it seems like a better case for privacy leakage applications could be made for a face recognition data set, or a pedestrian recognition data set, or similar application. The image data sets considered don't make as good an argument for protecting privacy as the two non-image data sets.

1. other ML classifiers
2. other datasets like face recognition datasest


----------- Comments for the Authors -----------
Summary: a well written paper with a throrough analysis of membership inference attacks and corresponding defense mechanisms. The analysis uncovers what seems to be the most determining vulnerability that’s exploited by the said attacks. A new defense mechanism that attacks this vulnerability at an aim of closing its gap on the expense of learning accuracy is proposed. The approach of the paper is nice and the contribution is considerable and the experiments are fair for their purpose. 
I only would suggest a careful proof reading of the paper as it contains several typos.

1. proof reading

----------- Comments for the Authors -----------
The paper deals with membership inference attacks, which pose a real
threat to many learning-based systems in practice. The authors first
provide a useful and comprehensive overview of a large number of MI
attacks and compare them on five different datasets that are also
commonly used in the related literature. Throughout their experiments,
they confirm that the generalization gap of a classifier significantly
affects its vulnerability against MI attacks. While this insight is
not new and has already been shown by previous works, I appreciate the
effort that the authors have spent to confirm these findings, and I
also like the presentation of the results.

Based on these findings, the authors propose a defense that tries to
reduce overfitting and minimizes the differences in label confidence
between members and non-members. To this end, the authors add a
MMD-based regularization term to the loss function. The basic idea of
countering MI attacks with regularization is (again) not new. However,
the defense is well-described and shows slight improvements compared
to existing defenses in a number of experiments. To further increase
the usefulness of the paper to other researchers, it would be great if
the authors would make their code publicly available.

Overall, the comprehensive evaluation of several MI attack along with
various state-of-the-art defenses compensates for the limited novelty
that this paper provides.

1. what to say?

==> hyptheory.tex <==
\subsection{Membership Inference Attack as a Hypothesis Test}

We now show that MI attacks are essentially hypothesis tests over the distribution of the model $F^T$ output for the training and test datasets.

\begin{theorem}\label{thm:hyp}
Let $D_\text{Tr}$ be the training data, $D_\text{Te}$ be the test data, where $D_\text{Tr} \cap D_\text{Te} = \emptyset$, and $D_\text{A}$ be the data available to the attacker, comprised of a mixture of examples from $D_\text{Tr}$ and $D_\text{Te}$.
We further make the common assumption that $D_\text{Tr}$ and $D_\text{Te}$ come from the same distribution of examples ---{\em i.e.}, no domain adaptation is needed.
Let $x \in D_A$ be a random (uniform) sample from $D_A$ that we wish to perform a membership inference attack. 
Under this scenario, the membership attack is equivalent to rejecting the null hypothesis for $x \in D_A$:
\begin{align*}
\mathcal{H}_0 &: x \in D_\text{Te} \: , \\
\mathcal{H}_1 &: x \in D_\text{Tr},
\end{align*}
where $\mathcal{H}_0$ is the null hypothesis and $\mathcal{H}_1$ is the alternative hypothesis.
Assume the priors $P(\mathcal{H}_0)$ and $P(\mathcal{H}_1)=1-P(\mathcal{H}_0)$ are known, that is, we know the fraction of samples in the adversary dataset $D_A$ that are expected to come from the training dataset $D_\text{Tr}$.
Then, under the following conditions, the above hypothesis test leads to:
\begin{enumerate}
    \item[(a)] Assume the attacker has black-box access to $F^{(T)}$, 
    and suppose the attacker has access to $D_\text{Tr}^\prime = D_\text{Tr} \backslash \{x\}$ and $D_\text{Te}^\prime \subset D_\text{Te}$. Then, 
    \[
    K_T = \frac{P(\mathcal{H}_1 | F^{(T)}(x), \{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime  \},  \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime  \} )}{P(\mathcal{H}_0 | F^{(T)}(x), \{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime  \},  \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime  \} )}
    \]
    is the Bayes factor that example $x$ is in $\mathcal{D}_\text{Tr}$.
%
%
    \item[(b)] Assume the attacker has access to the model architecture and a training dataset $D_\text{STr}^\prime$ with the same distribution as $D_\text{Tr}$ and $D_\text{Te}$ and can train a shadow model over $D_\text{STr}^\prime$. Then, 
    \[
    K_S = \frac{P(\mathcal{H}_1 | F^{(T)}(x), \{F^{(S)}(x') : x' \in  D_\text{STr}^\prime  \},  \{F^{(S)}(x') : x' \in  D_\text{Te}^\prime  \} )}{P(\mathcal{H}_0 | F^{(T)}(x), \{F^{(S)}(x') : x' \in  D_\text{STr}^\prime  \},  \{F^{(S)}(x') : x' \in  D_\text{Te}^\prime  \} )}
    \]
    is the Bayes factor that example $x$ is in $\mathcal{D}_\text{Tr}$.
\end{enumerate}
The Bayes factor gives how more likely it is for the alternative hypothesis to be true ($\mathcal{H}_1$), $x \in D_A$, than the alternative ($\mathcal{H}_0$), $x \not\in D_A$.
\end{theorem}
%
%
%
The proof is in the Appendix.
%
Theorem~\ref{thm:hyp} shows that MI is heavily influenced by the priors $P(\mathcal{H}_0)$ and $P(\mathcal{H}_1)$, which in our setting is the fraction of the attacker's data $D_A$ that come from the target's model training data $D_\text{Tr}$. 
Throughout this work we assume $P(\mathcal{H}_0) = P(\mathcal{H}_1) = 1/2$ to simplify our exposition, {\em i.e.}, we assume half of the $D_A$ samples comes from $D_\text{Tr}$.


Theorem~\ref{thm:hyp} also shows that the MI problem is closely related to the unsupervised learning task of  clustering in mixture models~\cite{raftery1996hypothesis}.
To see how mixture model clustering is related, consider applying Bayes rule
    \begin{align*}
    &P(\mathcal{H}_1 | F^{(T)}(x), \{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime  \},  \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime  \} ) \\
    &\propto P(F^{(T)}(x) | \{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime  \},  \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime  \} \mathcal{H}_1)P(\mathcal{H}_1| \ldots) \\
    &\propto P(F^{(T)}(x) | \{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime\}, \mathcal{H}_1)P(\mathcal{H}_1|\ldots),
    \end{align*}
where $P(\mathcal{H}_1|\ldots) = P(\mathcal{H}_1|\{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime  \},  \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime  \})$,
which is the probability of generating a probability vector $F_x = F^{(T)}(x)$ given we already observed  $\{F^{(T)}(x') : x' \in  D_\text{Tr}^\prime\}$ from the same generative model tied to $\mathcal{H}_1$. 
A similar equation on $\mathcal{H}_0$ gives 
\[
P(\mathcal{H}_0 | F^{(T)}(x),\ldots) \propto P(F^{(T)}(x) | \{F^{(T)}(x') : x' \in  D_\text{Te}^\prime\}, \mathcal{H}_0)P(\mathcal{H}_0),
\]
for the generative model tied to $\mathcal{H}_0$.
%
%

Finally, $D_A$ comes from a mixture of the two clusters tied to $\mathcal{H}_0$ and $\mathcal{H}_1$.
By reducing the hypothesis test to a clustering problem under a mixture of two models, we have given an underlying theoretical foundation of existing {\em Class-vector}, {\em Instance-vector}, {\em Global-loss}, {\em Global-probability}, {\em Global-topthree}, {\em Global-topone} attacks. 
These are all essentially clustering methods.
This insight helps explain the connection between identifiability and the generalization gap.


Firstly let's discuss the membership inference for a specific class using only the probability for the correct label and this probability follows a Beta distribution. 

Given a set $D$ of training data, a model $M$ training from it, and a set $T$ of test data.  $M: D \rightarrow P$. 

Let $P_D$ be the set of confidence vectors that $M$ outputs on instances in $D$, and $P_T$ be the set of confidence vectors that $M$ outputs on instances in $T$.  We assume that $P_D$ and $P_T$ can be viewed as samples from a Dirichlet distribution. 

Consider $C_D$, the set of confidence values that $M$ outputs on the correct label of instances in $D$, and $C_T$, the set of confidence values that $M$ outputs on the correct label of instances in $T$. 
$C_D$ and $C_T$ can be viewed as sampled from Beta distributions.  

Let $f$ denote the Beta distribution that $C_D$ is sampled from and $g$ denote the Beta distribution that $C_T$ is sampled from. 


The distribution of confidence vectors is Dirichlet distribution and the marginal distribution of a Dirichlet distribution is a Beta distribution. We denote the Beta distribution of members as $f$ and the Beta distribution of non-members as $g$. We denote the CDF of $f$ as $F$, the CDF of $g$ as $G$ and the intersection of $f$ and $g$ is $t$, i.e. $f(t) = g(t)$. Figure \ref{fig:beta_example} shows an example of $f$ and $g$. Generally we have $E[f]>E[g]$ since the trained model will be more confident on members than non-members. For attackers, the best attack strategy given these two beta distributions is that when the probability is lower than $t$, then this instance is predicted to be a non-member. If the probability is higher than $t$, then this instance is predicted to be a member. The attack accuracy can be calculated by this: 
\begin{equation}  
  \begin{array}{l}
    accuracy = \frac{G(t)}{G(t)+F(t)}*\frac{(G(t)+F(t))}{2} + \\
    \frac{1-F(t)}{1-G(t)+1-F(t)}*\frac{1-G(t)+1-F(t)}{2} = \frac{1+G(t)-F(t)}{2}
    \end{array}
\end{equation}
and the attack advantage is $\frac{G(t)-F(t)}{2}$. 

\begin{figure}
    \centering
    \includegraphics[width=6cm,height=6cm]{figures/pdf.png}
    \caption{pdf illustration.}
    \label{fig:beta_example}
\end{figure}

Next we need to consider how to calculate the generalization gap. We assume that the model is well calibrated and then the generalization gap is $E_f[x]-E_g[x]$. In summary, we need to prove that $E_f[x]-E_g[x]>\frac{G(t)-F(t)}{2}$. 

We know that $E_f[x] = \int_{0}^{1} f(x)x dx $ and we can rewrite this equation to be $E_f[x] = \int_{0}^{1} (1-F(x))dx$. Then the above equation could be rewritten as: $\int_{0}^{1} (G(x)-F(x))dx > \frac{G(t)-F(t)}{2}$.

Here we assume that there will only be one cross between $f$ and $g$, which is $t$ mentioned above. Since $f$ and $g$ are monotonic, $g(x)>f(x)$ when $x<t$ and $G(1)=F(1)=1$, we know that $G(x)-F(x) \geq 0$ holds for all $x \in (0,1)$. This means that $G(t)-F(t)$ is the max value for $G(x)-F(x)$ on $[0,1]$.

Now we need to prove that, the integration of $G(x)-F(x)$ on $[0,1]$ is larger than the half of its maximum value on $[0,1]$. This equation holds when $G(x)-F(x)$ is concave and $g(0)-f(0)>0$. 

\noindent Problem 1: How to prove this equation $E_f[x]-E_g[x]>\frac{G(t)-F(t)}{2}$ with $E_f[x]-E_g[x]$ ? \\
Problem 2: How can we generalize the above statements? \\
Problem 3: It is not possible to prove our guess using the maximum probability of the confidence vector, since there is no closed form distribution for the maximum of a dirichlet distribution.

==> rebuttal.tex <==

We emphasize that the main goal of this paper is to develop defenses against MI attacks.  We do not claim as contribution that Instance-Probability is a more practically effective attack.  The main contributions in this paper are: 1.the quantitative relationship between generalization gap and best attack advantage. 2. the proposed defense by reducing the gap.  To establish these contributions, we need to consider strong attacks, including computationally expensive ones.  As SOTA attacks essentially exploit the probability of the correct label, we introduced the Instance-Probability attack, which chooses a different threshold for each instance instead of one global threshold.  Results demonstrate that it is significantly more effective when defense mechanisms are deployed. 

Cost of different attacks

We will add computational cost analysis of different attacks.  It is true that Instance-Vector [19] and Instance-Probability [this paper] require more shadow models and are more expensive. 

Summary of attacks' performance

Table 2 on Page 8 shows the attack advantages of attacks considered in our paper for different datasets.  For CIFAR-10 and CIFAR-100, the numbers are averaged over all models.  We will make Figure 2 clearer by moving the legends as one row on the top, plotting generalization gap as a line across (instead of a bar), and adjusting the y-scale so that differences are clearer.

Performance of the new (Instance Probability) attack

This is discussed on Page 9, right column, the paragraph starting with "The Instance-Probability attack". 

Shadow model in defense

The shadow models are built in the exactly same way as the target models, i.e., the attacks are adapted to the defense.  We will clarify this in the paper.

Formal guarantee of defenses

Other than differential privacy, existing defenses also do not provide formal guarantee. In our opinion, provable guarantee must be balanced with testing accuracy.  Any defense that results in significant decrease in accuracy will not be used.  As shown in [15], DP-SGD provides worse tradeoff than Mem-Guard.  Our defense provides stronger privacy than Mem-Guard for the same accuracy. When revising the paper, we will add an experiment directly comparing our defense and defenses such as DP-SGD.

==> revise_suggestions_from_reviews.tex <==
 Review A:


##Question on Validation Set. 

-- we need to clarify the details of validation set.

We ensure that the validation set is disjoint from the training set of any target or shadow model and the evaluation set for MI attacks.  Each dataset we use comes with a training set $D$.  Effectively, we split D into 4 disjoint parts: $D_E$, $D_G$, $D_H$, and $D_V$.  To enable experiments where target models are trained with sets of different sizes, each target model is trained using randomly selected half of $D_E$ and additional instances from $D_G$ to reach the desired training size.  Shadow models are training using randomly selected half of $D_E$ and additional instances from $D_H$.  Instances in $D_E$ are used for evaluating MI attacks.  Validation sets are randomly selected from $D_V$, and has the same number of instances as the training size.  Specifically, for each class, the number of instances is also the same. 

##On Assumptions.

-- assumptions that the test set is balanced are borrowed from previous papers. maybe we need to add more comments on what is going to happen when the assumptions do not hold.

%Indeed our evaluation setting implicitly assumes that half of the instances are drawn from the training set, which makes the number of members and non-members the same.  Most previous papers on MI [15,24,25,31] use this setting.  We choose to follow previous work to use this setting because it enables immediate comparison with the state of the art.  

The issue whether some subgroups may be more susceptible to MI attacks is interesting, and largely beyond the scope of this paper.  We will add discussion on this and other caveats as suggested.  In our proposed defense, we calculate the MMD loss for each class instead of the whole distribution, which should help ensure that MI attacks for instances belonging to each class are protected against. Note that we only care about membership information of actual instances that could be used in the training dataset.  For an artificial instance that falls outside the training distribution, one may be able to conclude that it is a non-member, but that is not a privacy threat if the instance does not correspond with any actual instance.  

%Regarding the assumption on how the attack works, we did not start with any assumption.  We started by implementing promising attacks that we can find in the literature (Section 2.2), and then coming up with new attacks that we feel may be more effective.  In fact, some of the attacks we tried are not discussed in the paper because they turned out to be less effective.  Some of the attacks use the full prediction vector.  However, based on experimental results, we found that simply using the probability of the true label can give similar attack accuracy as using the full prediction vector, therefore we conjecture that the probability of the true label is the most important feature for MI attacks.  When that is the case, the best MI advantage becomes closely related to g.  Furthermore, the attack advantage of the baseline attack is strictly related to g.  

%We have performed some mathematical analysis on why g is closely related to MI advantages.  When assuming that the model's probability distribution for the correct label follows beta distribution where the parameters in certain ranges, g is related to the best MI attack accuracy from hypothesis testing.  Empirically the distributions from NN models we observe satisfy the assumptions, as can be seen from Figure 5 (in the appendix).  However, one could legitimately challenge whether the assumptions are valid.  We hence did not include that analysis and focus on purely empirical support.  However, this analysis does increase our confidence that the bound broadly holds. 

##About Methodology.

-- add the experiments on running MI on the validation set. 

In the submission, we did not run the membership inference on the validation set.  Since the model is not directly optimized over the validation set, we do not expect MI attacks to be effective.  Over the last few days, we conducted MI attacks on instances used in the validation set for MMD training and found that all existing MI attacks are ineffective against them.  We will add these results to the paper.  

Our conjecture that the power of an MI attack is upper-bounded by g is limited to black-box MI attacks. There is certainly the possibility that a more effective black-box MI attack is discovered and falsify our conjecture. However, due to the mathematical analysis mentioned above, we think this is unlikely for mainstream NN datasets.  If the adversary is allowed to have white-box access, more effective attacks may be able to find.  That is one direction we plan to investigate in the future. 


1. On the figures, we did mean percentage points.  We will clarify that. 
2. Paper [25] simply shows that the attack advantage is higher when the gap is larger.  Our contribution is that we observed a quantitative relationship between attack accuracy and the gap, and we developed new defenses utilizing this observation.


Review C:
1. ignores attack that does not rely on generalization gap[20] 

-- need to consider the indirect attack in [20]

2. should add more details to the weights of MMD loss

-- more comments on how to tune the weights?

Review D:

1.Missing intuition behind the choice of g as the upper bound 

-- ?

2.Models are trained on subsets of the data, with artificially-induced generalization gaps favoring membership inference

-- we have ablation study on training set size.


5.Perhaps consistently studying the impact of training set sizes on different aspects evaluated (rather than treating the dataset size as a separate evaluation point) would help appreciate some of the claims made.

-- more experiments regarding the training set size?

6. Given that improving generalization is the underlying goal of most ML techniques, is a defence that improves generalization saying that we are trying to obtain a better performing model? Furthermore, if we compare the drops in attack advantage reported in Section 4.4 with those measured by increasing training set size in 4.3, the defence does not seem to provide significant gain. Is there a qualitative difference in the effect of the proposed techniques on models when compared to other regularizers aimed at improving the model's generalization?  

-- Maybe we need to add something comparing with other regularizations. ??? 


Review E:

Also, see other datasets in "ML-Leaks: Model and Data Independent Membership Inference Attacks and Defenses on Machine Learning Models". 

-- we use Location in our paper. UCI Adult is not attackable (the best attack advantage is really small). For datasets used in ML-leaks, maybe we want to add more experiments.

Why did Mix-up training fail for Purchase and Texas datasets? This needs an explanation, otherwise why is this a viable defense? 

-- (4) why mix-up fail on purchase and texas?

* How would the proposed defenses work in a white-box setting? A discussion would be useful.

-- what should be added?


==> revision_ndss.tex <==
1. pseudocode for defense

2. more discussion of the novelty of the new defense because it sounds incremental by now

3. grammar errors and improve writing

5. Probability-vector oracle model is the most explored model, but not the most natural model? -- change to ``most explored'' ?

6. more discussion on why just using the prob of the correct label can achieve best acc

7. more discussion on attacks?

8. Figure 3,4,5,6 and table 4,5 needs more discussion.

9. moving parts of the analysis on known attacks/defense to appendix? and more discussion on comparing our defense with other works.

10. need to compare with other regularizers // what to compare?

11. compare with knowledge distillation // bad testing accuracy. not compatible with mix-up

12. mix-up with dp // collecting data. seems to be similar to MMD+mix-up

13. Compare with adversarial regularization or knowledge transfer // no need to compare with adversarial regularization. compared with knoledge transfer in 11

14. overfitting on validation data -- discussed

15. compare with L2 + dropout .. In normal training -- normal training already used L2+dropout. Have the data for model trained without L2 and dropout.

16. add more related works in the end.

17. comparing dp with mmd on purchase and texas  // MMD is better!


